A Unified View of Delta Parameter Editing in Post-Trained Large-Scale Models

Post-training has emerged as a crucial paradigm for adapting large-scale pre-trained models to various tasks, whose effects are fully reflected by delta parameters (i.e., the disparity between post-trained and pre-trained parameters). While numerous studies have explored delta parameter properties via operations like pruning, quantization, low-rank approximation, and extrapolation, a unified framework for systematically examining these characteristics has been lacking. In this paper, we propose a novel perspective based on Riemann sum approximation of the loss function to elucidate delta parameter editing operations. Our analysis categorizes existing methods into three classes based on their post-editing performance: competitive, decreased, and improved, explaining how they are expressed by the Riemann sum approximation term and how they alter the model performance. Extensive experiments on both visual and language models, including ViT, LLaMA 3, Qwen 2, and Mistral, corroborate our theoretical findings. Furthermore, we introduce extensions to existing techniques like DARE and BitDelta, highlighting their limitations in leveraging the properties of delta parameters and reorganizing them into general expressions to enhance the applicability and effectiveness of delta parameter editing in post-trained models.

==> Bakckups/Introduction.tex <==
% 一句话总结：我们对post training后参数变化进行了探究，发现了对于post training模型的近似等价空间，并通过一个简单的公式对经验性的进行了总结。
\section{Introduction}

% 第一段：pretraining-posttraining 已经成为了现在深度学习的重要范式
% 分论：
% - 在 BERT/ViT 上 finetuning 模型可以让模型使用少量数据学习特定任务的能力；
% - 在 LLM 上，SFT 和 RLHF 使得 LLM 与人类行为对其。

With the remarkable success of large-scale pre-trained models, post-training has emerged as the de facto standard paradigm for effective adaptations to various tasks \citep{DBLP:journals/corr/abs-2403-14608,DBLP:journals/corr/abs-2402-02242,DBLP:journals/corr/abs-2002-06305,DBLP:journals/corr/abs-2303-18223}. Conceptually, post-training optimizes the parameters of pre-trained backbone on task-specific data, endowing models with diverse abilities like visual recognition \citep{DBLP:conf/nips/ChenGTWSWL22,DBLP:conf/cvpr/0002ZV022}, instruction following \citep{DBLP:conf/nips/RafailovSMMEF23,DBLP:journals/corr/abs-2402-01306}, and mathematical reasoning \citep{DBLP:journals/corr/abs-2308-09583,DBLP:journals/corr/abs-2407-13690}. It has been noted that the impact of post-training is fully manifested in the \textit{delta parameters}, which are defined as the difference between parameters of pre-trained and post-trained models \citep{yu2023language}. 

Due to the inherent correlations between delta parameters and post-training, 

In recent years, there is a trend on studying the role of delta oarameters

% In recent years, the pre-training \& post-training paradigm has emerged as a cornerstone in deep learning, revolutionizing the way models are developed and applied across various domains. 
% This two-stage approach, which involves pretraining on large-scale datasets followed by task-specific fine-tuning or adaptation, has demonstrated remarkable effectiveness in enhancing model performance and generalization capabilities.
% Notably, this paradigm has shown significant success in two key areas:
% (1) fine-tuning pretrained models like BERT for natural language processing and Vision Transformers (ViT) for computer vision, enabling the acquisition of task-specific knowledge with limited labeled data;
% and (2) applying techniques such as Supervised Fine-Tuning (SFT) and Reinforcement Learning from Human Feedback (RLHF) to align Large Language Models (LLMs) with human preferences and behaviors. 
% While the effectiveness of posttraining is evident, a systematic understanding of how parameter changes during this process contribute to performance improvements remains elusive.

% 总结句：posttraining 对模型参数的影响是很小的，但能取得如此好性能的原因仍然是未知的。现在逐渐有一些研究将视野聚焦在 posttraining 的参数变化 delta 上。
% （这样写有一个问题：我们最终的结论也没有说明 posttraining 如何靠小参数实现好性能，可能需要换一句）
% 分论：
% - BitDelta 发现保持 delta 参数的符号不变，将所有的值都替换成一个值，模型的大部分性能可以保持；
% - Dare 发现将 delta 参数中的 k%置为 0，将剩下 1-k%的参数乘 1/（1-k%）后，模型性能基本可以保持不变。
% 这些研究展现出了 delta 参数的具体的值、部分完整参数可能是冗余的，但是仍然没有研究对 posttraining 过程中的参数进行系统研究。

Recent research has begun to explore the nature of parameter changes (\textit{delta}) during posttraining, revealing intriguing properties that challenge our understanding of model adaptation.
% 修改：下面3句合成一句
These findings suggest that the specific values or completeness of delta parameters may be partially redundant.
% For instance, BitDelta~\citep{} have shown that preserving only the sign of delta parameters while replacing their magnitudes with a constant value can largely maintain model performance.
% Similarly, Dare demonstrated that setting a portion of delta parameters to zero and scaling the remainder can yield comparable results to the original instruct model.
However, a comprehensive framework for systematically analyzing and characterizing the parameter changes during posttraining is still lacking, leaving a significant gap in our understanding of this crucial process.

In this study, we discover that the signs of the delta parameters plays a crucial role in post-trained models.
We initial observe that xxx.
% 更近一步，We find that 存在一个与post-trained models近似等价的群，这个群里的矩阵与delta的差值正交。
% 群中两种元素：
% 1. 对称：。
% 2. 非对称：。

% 第四段
% 实验上的架构/task

% 第五段
% contribution

% 2.1 prelim
% xxx 1: value不重要
% xxx 2: 整体是对称的

% 2.2 对称
% xxx 3: 符号变化，rescale

% 2.3 不对称
% xxx 4: 
% xxx 5: 

% 2.4 general
% 1:更近一步，We find that 存在一个与post-trained models近似等价的群，这个群里的矩阵与delta的差值正交。

% 3. 实验
% 4. 解释
% 5. application
% 相关bitdelta/dare
% 6. related work
